Why Does a Visual Question Have Different Answers?

Visual question answering is the task of returning the answer to a question about an image. A challenge is that different people often provide different answers to the same visual question. To our knowledge, this is the first work that aims to understand why. We propose a taxonomy of nine plausible reasons, and create two labelled datasets consisting of ~45,000 visual questions indicating which reasons led to answer differences. We then propose a novel problem of predicting directly from a visual question which reasons will cause answer differences as well as a novel algorithm for this purpose. Experiments demonstrate the advantage of our approach over several related baselines on two diverse datasets. We publicly share the datasets and code at https://vizwiz.org.

==> mapping.tex <==
{\color{blue}

\begin{figure*}[!tbhp]
\captionsetup[subfloat]{farskip=-1pt,captionskip=-1pt}
\centering
\includegraphics[clip=true, trim=0 492 0 0, width=0.99\linewidth]{diag/dis-source-solutions-mapping.pdf} %trim - left, bottom, right, top
\hfill
\caption{
Schematic diagram of our proposed visual question answering system, which recruits several existing solutions to mitigate answer disagreement.
}
\label{fig:soln_mapping}
\end{figure*}

\section{Proposed Visual Question Answering System}
\label{sec:mapping}



Various solutions exist to resolve crowd disagreements that arise due to different reasons. 
Yet, currently a system designer has no way of knowing which solution(s) to apply, without first reviewing the VQ with answers, and then identifying the reason(s) for which the disagreement occurred. 
Using our proposed taxonomy, a trained VQA system will be able to detect which specific reason(s) will cause disagreement(s) to occur, and thereby recruit appropriate disagreement resolution solution(s). 
We present such a VQA system in \textbf{Figure \ref{fig:soln_mapping}}, and explain its working below.



Using a smartphone app, a user asks a visual question by snapping a photo, and asking a spoken question about it.
The app captures a burst of image frames, including frames before and after the camera button is tapped by the user \textbf{(Figure \ref{fig:soln_mapping} (a))}, and performs two image-based operations, Steps $I_1$ and $I_2$. %, on these images.
In $I_1$, the system calculates the ``image specificity'' (i.e. whether the image will elicit a converging textual description) \cite{jas2015Imagespecificity} of each image in the burst, and selects the image with highest specificity. 
$I_2$ takes the image chosen by $I_1$, and performs a host of image-enhancements. 
These include up-sampling the image if it is below a threshold resolution \cite{dong2016image, shi2016real, ledig2017photo},
correcting motion blurs \cite{sun2015learning, kupyn2018deblurgan} and blurs due to camera-shakes \cite{nah2017deep},
and overall image enhancements such as improving contrast, brightness, and dynamic range \cite{hasinoff2010noise}.
This produces the final candidate image \textbf{(Figure \ref{fig:soln_mapping} (c))}.
Thus, by selecting the most specific image, $I_1$ helps to resolve camera framing errors and ambiguity errors in the image (AMB), while $I_2$ resolves issues due to low quality (LQI).

Meanwhile, the spoken question from the user is transcribed into textual form \textbf{(Figure \ref{fig:soln_mapping} (b))}.
In Step $Q_1$ this text is passed through state-of-the art solutions for grammatical error correction (e.g. \cite{yuan2016grammatical, xie2016neural, dahlmeier2011grammatical}) which can help to transform an invalid question (INV) into a grammatically valid sentence or question \textbf{(Figure \ref{fig:soln_mapping} (d))}.
Then the question is passed through Step $Q_2$, which tries to eliminate ambiguity (AMB) in the question text using solutions like \cite{kovashka2015Discoveringattributeshades, jurgens2013embracing}, and produces the final unambiguous, valid question \textbf{(Figure \ref{fig:soln_mapping} (e))}.

The final image \textbf{(Figure \ref{fig:soln_mapping} (c))} and the question \textbf{(Figure \ref{fig:soln_mapping} (e))} are then presented as input to a disagreement-source prediction model $M$.
Since LQI, AMB and INV have already been resolved, the model $M$ places special emphasis to detect IVE, SBJ, DFF or no disagreement.
If IVE is predicted (i.e. answer to the question is not present in the image), the user is asked to create a new visual question.
However, if SBJ or DFF is predicted, the user is warned that possible answer disagreement can arise, and is given the choice  to ask a new question, or go ahead with the current question \textbf{(Figure \ref{fig:soln_mapping} (f))}.
If the user chooses to continue with the current visual question, the system goes into the answer collection stage \textbf{(Figure \ref{fig:soln_mapping} (g))}.

The actual answering of the  visual question can happen either via crowdsourcing, or by another artificial intelligent system (which is beyond the scope of this work).
Having collected one or more answers \textbf{(Figure \ref{fig:soln_mapping} (h))}, they are first passed through Step $A_1$, which performs spam-filtering \cite{vuurens2011much, eickhoff2013Increasingcheatrobustness, vuurens2012obtaining, gadiraju2015Understandingmaliciousbehavior}.
The non-spam answers \textbf{(Figure \ref{fig:soln_mapping} (i))} are then subjected to Steps $A_2$ and $A_3$.
$A_2$ involves reducing answer-disagreement due to synonyms (SYN).
For this purpose, a dictionary of synonyms can be maintained along with a ``base'' word.
When a synonym occurs in the answers, it is internally translated to the base word.
E.g. whenever a synonym for the word ``round'' occurs in the answers (such as ``circular'', ``disk-shaped'', ``spherical'', ``ball-shaped'', etc.) it will be converted to the word ``round'' in the background, and answer-convergence will be achieved.
Additionally, algorithms for measuring semantic similarity of words, such as
word2vec \cite{mikolov2013distributed} and GloVe \cite{pennington2014glove}, can also be used to determine if two words are similar in meaning.

Step $A_3$ tries to minimize answer-disagreement due to granularity (GRN), by pairwise comparing the answers using solutions like sent2vec \cite{pagliardini2017unsupervised}, and Universal Sentence Encoder \cite{cer2018universal}, to see if all the answers are semantically similar (i.e. whether they present the same general idea).
Finally, $A_3$ outputs the answer(s) to the visual question asked by the user \textbf{(Figure \ref{fig:soln_mapping} (j))}.


% Low Quality Images (\underline{LQI}) occur due to poor resolution, camera framing error, or lack of focus. 
% Solutions like blur detection and correction \cite{liu2008image, sieberth2016automatic}, 
% image-sharpening \cite{muller1974real, parulski1997automatic, schavemaker2000image}, 
% % automated detection of image quality \cite{ribeiro2011crowdsourcing},
% and tools supporting blind photography \cite{jayant2011supporting} (esp. for \textit{VizWiz})
% can be applied in this scenario.
% For invalid questions (\underline{INV}), solutions include question-text processing \cite{strzalkowski2006advances}, followed by automated techniques for grammatical error detection \cite{de2008classifier} and correction \cite{dahlmeier2011grammatical}.
% Difficult visual questions (\underline{DFF}) can be tackled  by combining methods for assessing difficulty of textual questions \cite{bachrach2012grade} and difficulty of image annotation tasks \cite{welinder2010multidimensionalwisdomcrowds}.
% Ambiguity (\underline{AMB}) can be handled using solutions proposed for measuring image specificity (i.e. whether an image elicits a converging textual description from the crowd) \cite{jas2015Imagespecificity}, and for determining the different shades of meaning present in textual product label attributes \cite{kovashka2015Discoveringattributeshades}.
% Subjectivity (\underline{SBJ}) can be modelled and resolved by techniques proposed by \cite{wan2016modeling, nguyen2016Probabilisticmodelingcrowdsourcing}.
% Synonymous answers (\underline{SYN}) due to using different words having same meaning, or due to spelling errors, can be detected and corrected using methods described by \cite{clements2008detecting, futagi2008computational, baker2011identifying}.
% Lastly, spam answers and malicious behaviour of crowdworkers (\underline{SPM}) are discussed at length by \cite{vuurens2012obtaining, gadiraju2015Understandingmaliciousbehavior}, 
% while solutions for spam prevention and resolution are proposed by \cite{vuurens2011much, eickhoff2013Increasingcheatrobustness}.

}










% Various solutions exist for resolving these disagreements, yet, currently a system designer has no way of knowing which method(s) to apply without first reviewing the VQ with answers to figure out the reason disagreement occurred.
% Using our proposed taxonomy, a ideal smart VQA system will be able to detect which specific reason(s) will cause disagreement(s) to occur, and thereby recruit appropriate disagreement resolution solution(s). 
% For instance, LQI

% Our work fills this gap by 
% (1) establishing a taxonomy of causes that can lead to disagreement and 
% (2) providing a large-scale dataset for training machines to detect the cause for a given VQ. 
% Then, given a VQ at test time, the trained machine can detect which reason(s) will cause disagreement(s) to arise, and so recruit appropriate disagreement resolution method(s). e.g. apply [31] when the machine detects AMB is the problem. We will clarify this mapping between our disagreement causes and existing solution(s).

==> prediction-system-old.tex <==
\section{Predicting Why Answers Differ}
\label{sec:ml}
Having seen that answer disagreements can arise for different reasons, we next explore a novel problem of predicting why the answers will differ, given the QI pair and optionally the answers.
We introduce two machine learning models, and describe the experiments to assess their accuracy in making predictions.



\subsection{Machine Learning Setup}
\label{sec:ml_setup}

\subsubsection{\textbf{Problem Definition and Evaluation:}}
\label{sec:ml_evaluation}
We pose the task of predicting answer-disagreement-source(s) as a multi-label binary classification problem. 
The input is a QI pair and optionally the crowdsourced answers.
The output is a binary value for each of the 10 disagreement-source labels, indicating whether that label is the reason for answer-disagreement of the VQ.
In other words, we consider each disagreement label as a distinct binary classification problem.
We evaluate each classifier using a precision-recall curve, and the average precision score.


\subsubsection{\textbf{Ground Truth:}}
\label{sec:ml_gt}
We compute binary ground truth labels for all the 10 disagreement-source labels for each VQ.
Specifically, we examined the five crowdsourced labels per VQ, and considered a disagreement-source label as `1' (i.e present), if at least two people selected that label.
%agreed that reason occurred.
The 2-person threshold is a reasonable choice when five answers are crowdsourced, as indicated by \citep{bragg2013crowdsourcing, little2009turkit}.
% , as it is neither too loose as `trust-all', nor too restrictive as `trust-majority'.

\begin{figure*}[!hbtp]
\captionsetup[subfloat]{farskip=-1pt,captionskip=-1pt}
\centering
\includegraphics[clip=true, trim=0 275 0 0, width=0.9\linewidth]{plot/pr_curve_rf.pdf} %trim - left, bottom, right, top
%\hfill
\caption{
% Precision-recall of the predictions made by our
Performance curves of our random forest model, for (a) \textit{VizWiz} and (b) \textit{VQA\_2.0} datasets.
The legends show average precision scores of our model (left), and \textit{Status Quo} baseline (right), for each label.
% Due to high class imbalance in the training data, and relatively low size of dataset (20,000 for training), the neural network model was not able to generalize effectively, and performed no better than the \textit{Status Quo} baseline.
}
\label{fig:pr_curve_rf}
\end{figure*}

\subsubsection{\textbf{Train/Validation/Test Split:}}
\label{sec:ml_split}
We used the whole \textit{VizWiz} dataset, including the QI pairs where all answers were identical (i.e., 3\% of the total VQs) to grow the size of the training set.
Employing the train/validation/test split from \cite{Gurari_2018_CVPR}, we have 20,000 training (65\%), 3,173 validation (10\%), and 7,988 test (25\%) samples.  For the 5,031 VQs from the \textit{VQA\_2.0} dataset, we introduced a 65/10/25 split which resulted in 3,230 training, 513 validation, and 1,291 test examples.

% as well as to partially correct for the class-imbalance present in our data (Section~\ref{sec:lbl_freq})


\subsubsection{\textbf{Baseline:}}
\label{sec:ml_baselines}
To the best of our knowledge, no prior work has tried to predict the reason(s) why a VQ will have different answers.
So the best option available today is to randomly guess the reasons.
Thus, we compare our system against a \textit{Status Quo} predictor, which randomly assigns a binary value for each of the ten disagreement-labels, to simulate random guessing.

\subsection{Machine Learning Models}
\label{sec:ml_impl}

\subsubsection{\textbf{Random Forest:}}
\label{sec:ml_rf}
We proposed a random forest~\cite{breiman2001random} model.  We chose to extract features that describe the image, question, and 10 answers.  

As \underline{\textit{image features}}, we use the Computer Vision API\footnote{https://azure.microsoft.com/services/cognitive-services/computer-vision/} from Microsoft Cognitive Services to extract:
%The `analyze' module of the Computer Vision API outputs information about an image's visual content.
%, like allocated tags, prominent colours, number of faces detected, whether the image is adult or racy, etc.
(a) number of category labels assigned to the image (`outdoor', `abstract', `food', etc),
(b) number of tags assigned to the image (`pizza', `sign', `water', `television', etc.),
(c) number of distinct colours detected in the image, %(both dominant colours and accent colours),
and
(d) number of faces detected in the image.
Intuitively, the number of categories and tags associated with an image informs two things:
(1) the number of different ways an image can be interpreted (e.g. `sitting at a table' versus `eating'), %thus giving a measure of ambiguity,
and
(2) the number of objects in an image competing for an person's attention.
When an image is assigned multiple tags like `sitting at a table' and `eating', then a question of the form `What is the person doing?' will be considered ambiguous (AMB), as the answer could either be `sitting' or `eating' or both.
Also, if an image is associated with a number of categories and tags, it indicates there are multiple salient objects in the image competing for the viewer's attention.
Therefore, answers to `What is this?' questions will result in a variety of answers, depending on which object attracts the viewer's attention.
This will give rise to synonyms (SYN) and varying granularity (GRN) in the answers.
%thereby informing about answer granularity and synonyms, as the more the number of salient objects in the image, the more different will be the level of details expressed in the answers.
% We also included number of colours, as we saw in Section \ref{sec:lbl_freq} that seeking colour-related information often leads to disagreement (in 93\% cases).


For \underline{\textit{question features}}, we considered the following:
(a) number of words in the question, as from Section \ref{sec:amb_syn_grn} we saw that lengthy questions tended to be ambiguous, (especially for \textit{VQA\_2.0}),
(b) whether the word `colo(u)r' is present in the question, as a binary label, 
and
(c) the most common answer-type from the 10 crowdsourced answers
\cite{gurari2017CrowdVergePredictingIf, Gurari_2018_CVPR}, namely numeric, yes/no, other, unanswerable. %, as four binary labels: `Ans Numeric?', `Ans Yes/No?', `Ans Other?', and `Unanswerable?'.
% These labels come from the dataset \cite{gurari2017CrowdVergePredictingIf}
Intuitively, the most common answer-type can indicate whether answer disagreement can occur.
For instance, a generic `other' question has more chance to produce a wide variety of answers, than a `yes/no' question.

For \underline{\textit{answer features}}, we counted the number of words in each of the ten answers, as difference in the number of words indicates a difference in the answer text.

We used the random forest implementation of Scikit-Learn \cite{scikit-learn}, with 1,000 trees, `balanced' class-weights (so that all output labels get equal priority, despite class imbalance in training data), and maximum tree-depth of 20.


%A random forest classifier is formed by collating the outputs of multiple decision trees (via an ensemble process), and forming a prediction.
%The randomness in a random forest arises from two aspects:
%(a) the trees train on only a random subset of the training data, i.e., no tree sees the full training set, and
%b) the trees use a random subset of the input features to make a prediction, i.e. none of the trees examine all the input features.
%These randomness criteria helps the trees to learn about different aspects of the training data with slightly different perspectives, and it is expected that ensembling the output from all trees will result in a better prediction than that of a single decision tree alone.


%%%%%%%%%%%%%%%%%% result_rf %%%%%%%%%%%%%%%%%%
\begin{figure*}[!thbp]
\captionsetup[subfloat]{farskip=0pt,captionskip=4pt}
\centering
\includegraphics[clip=true, trim=0 150 200 0, width=\linewidth]{diag/result_rf_feature_imp.pdf} %trim - left, bottom, right, top
\caption{
(a): Average precision scores of our random forest model, against the \textit{Status Quo} (random) baseline, for \textit{VizWiz} and \textit{VQA\_2.0} datasets.
% Performance of the random forest implementation of our model, 
% The values are average precision scores, considering the prediction of each label as a binary classification task.
The figures are for four ablations: training and testing on question, image and answer features (`QI+A'), %, row 1),
question and image features only (`QI'), %, row 2),
question features alone (`Q'), %, row 3),
and image features alone (`I'). %, row 4).
Italicized values with asterisk (*) indicate instances where our model performed worse than \textit{Status Quo}.
(b) - (g): Importance of our handcrafted features for predicting disagreement-sources, as returned by our random forest model, trained on `QI+A', `QI' and `Q', for the \textit{VizWiz} (b)-(d) and \textit{VQA\_2.0} (e)-(g) datasets.
Question, Image and Answer feature-names start with Q:, I:, and A\#: respectively.
}
\label{fig:result_rf}
\end{figure*}
%%%%%%%%%%%%%%%%%% result_rf %%%%%%%%%%%%%%%%%%



\subsubsection{\textbf{Deep Learning:}}
\label{sec:ml_nn}
Given the many successes of deep learning systems, we also developed a deep learning model for our prediction problem. 
We adapted our architecture from the hybrid neural network proposed in \cite{antol2015VqaVisualquestion}.
It takes as input the raw image, question, and (optionally) the 10 answers.  The text inputs are converted to numeric form using GloVE (Global Vectors for Word Representation) pre-trained 100-dimensional word embedding \cite{pennington2014glove}, which was trained on the entire text corpus of Wikipedia 2014.  Then they are passed through a 256-dimensional Long Short Term Memory (LSTM) \cite{gers1999learning} model.  The image is encoded using the popular VGG16 \cite{simonyan2014very} pre-trained vision model, which takes a 224 $\times$ 224 colour image as input, and outputs a 4096-dimensional vector.  The image and text encodings are then combined and passed through two fully connected layers with ReLu (Rectified Linear Unit) activation functions, and are finally output via a 10-node sigmoid activated output layer, corresponding to 10 probabilities for each disagreement-source label. % To overcome the problem of having a relatively small amount of training data (e.g., 23,000 samples), we froze the pre-trained layers and used a low learning rate.  %We used the Keras framework \cite{chollet2015keras} with TensorFlow backend \cite{tensorflow2015-whitepaper} to implement our model.



\subsection{Performance Analysis}
\label{sec:ml_result}

\subsubsection{\textbf{Overall Performance:}}
\label{sec:ml_result_rf}
We first examine the performance of the models to predict the disagreement-source directly from the VQ and answers.  Figure \ref{fig:pr_curve_rf} shows the precision-recall curves for the proposed random forest model as well as the average precision scores for it and the \textit{Status Quo} approach.  As observed, the random forest model outperforms \textit{Status Quo} for most disagreement-causes.  

For the \textit{VizWiz} dataset, Ambiguity (AMB), Synonyms (SYN) and Granularity (GRN) are predicted with the highest average precision (Figure \ref{fig:pr_curve_rf}a).  
The model success appears to correlate with most frequent disagreement-sources in the dataset, probably because there are more training examples.
  

The model performs worst for detecting spam (SPM) for the \textit{VizWiz} dataset. Intuitively, this makes sense since a worker's choice to return bogus results is probably independent of the task at hand. Hence, we would not expect that information about the QI pair or the answers will help in deciding when a worker will submit spam.

While the model does demonstrate some predictive power for detecting difficulty (DFF) and subjectivity (SBJ), it is a less strong predictor compared to AMB, SYN and GRN. 
This is may be because detecting whether a question is difficult or subjective requires understanding the meaning of the question, which is possible through more sophisticated natural language processing and semantic analysis, rather than simple statistical features such as word count or presence of certain words like `colour'. 
Another reason for non-performance is possibly the lack of sufficient training examples (e.g. less than 10\% in \textit{VizWiz}).

For the \textit{VQA\_2.0} dataset, performance is similar to \textit{VizWiz} with respect to labels AMB, SYN, GRN, IVE, DFF, SPM and OTH.  Significant differences are observed for LQI and SBJ labels.  We hypothesize the diffence in LQI performance is due to the nature of the images themselves.  While images in \textit{VizWiz} are typically more blurred or ill-formed when they are LQI and so easier to detect, images from MS-COCO \cite{lin2014MicrosoftCOCOCommon} typically share with other images in the dataset that they are high photographic quality even when they are LQI.


%Thus, our \textit{VQA\_2.0} dataset contained less than 10\% VQs labelled with LQI (Figure \ref{fig:hist_lbl_freq}), and so our model did not have enough training examples LQI, and performed worse than the \textit{VizWiz} dataset.   

%The reason for better performance of SBJ in the \textit{VQA\_2.0} dataset goes to the label frequency imbalance of the datasets as well.
%SBJ occurs for about 20\% of the VQs in \textit{VQA\_2.0} dataset, while it occurs for only 5\% \textit{VizWiz} questions.
%Hence the model performs better on \textit{VQA\_2.0} dataset.

For completeness, we include the precision-recall curves for the deep learning model in the Supplementary Materials.  However, we exclude it from the main paper as the model was unable to perform better than \textit{Status Quo}.  We attribute the poor performance to the limited amount of training data and huge class imbalance.  Specifically, the relatively low number of training samples (20,000 as opposed to millions for large-scale systems) makes it difficult to effectively learn the weights necessary for this end-to-end machine-learning task.  This issue is compounded by the huge class imbalance of AMB, SBJ, and GRN, where a standard `yes predictor' for those three labels would already yield promising performance; i.e. predict AMB, SYN and GRN for all samples.  




\subsubsection{\textbf{Predictive Cues:}}
\label{sec:predictive_cues}

We also conducted ablation studies to investigate what cues are most predictive of the disagreement-source, using the top-performing random forest model.
Specifically, the four ablations we trained on are
(a) question, image and answer features (`QI+A'),
(b) question and image features only (`QI'),
(c) question features alone (`Q'), and
(d) answer features alone (`A').
% Results are shown in Figure~\ref{fig:result_rf}.  
We also report the importance of individual features in Figures \ref{fig:result_rf}(b)-(c). 
Specifically, it reveals the learned importance of each feature for three ablations of the model, across both datasets.
The importance values are obtained from the Scikit-Learn implementation of the random forest classifier. 
Specifically, we used the ``gini impurity'' criteria \cite{Breiman1984Classification}


Figure \ref{fig:result_rf}(a) shows the average precision results for these four ablations of our random forest model, and the \textit{Status Quo} baseline across both \textit{VizWiz} and \textit{VQA\_2.0} datasets.  Overall, reducing the number of input features causes a performance deterioration.  Still, except for `I', all variations perform better than \textit{Status Quo} for all the labels across both datasets.



As noted above, for the \textit{VizWiz} dataset, Ambiguity (AMB), Synonyms (SYN) and Granularity (GRN) are predicted with the highest precision.  This can be partially due to the high frequency of these labels in the dataset.
However, except for `I', all other variants perform significantly better than \textit{Status Quo} baseline.
It is interesting that even without the answer features, our model is able to predict answer related issues like SYN and GRN from `QI' and 'Q' features only.
This can be attributed to the features: number of image tags, number of image categories, and number of words in the question, as seen from Figures \ref{fig:result_rf}(c) - (d).
As we hypothesized, count of image tags and categories inform about the number of different salient objects in the image, and more objects lead to answers with synonyms and varying granularity.



Low Quality Image (LQI) and Insufficient Visual Evidence (IVE) are predicted fairly well by `QI+A', `QI' and `Q'.
We believe that the combination of the features: number of image tags, and count of words in the question, play a significant role here.
A question with low word count (e.g. 'What is this?') is probably not invalid by itself.
However, an image with low tag count is possibly blurred, or does not contain enough identifiable entities, resulting in LQI.
A combination of low tag count in image, and high word count in question suggests that IVE is about to occur.
Since the `Q' ablation performs better for these labels than `I', we believe that some other question features (like a combination of the four answer-type binary variables) may also play a role.
We hypothesize that the performance for LQI and IVE drops significantly for `I', since these additional question based features are not available.




We hypothesized in Section \ref{sec:lbl_freq} that a VQ seeking colour related information leads to particular disagreement-sources.
So we included the two colour related features: count of distinct salient and accent colours present in the image, and whether the word `colo(u)r' is present in the question.
Interestingly for both datasets, presence of `colo(u)r' is not as important as the number of colours present in the image (Figure~\ref{fig:result_rf}b,c,e,f).
This indicates that answer disagreement occurs with higher probability if many different colours are visible in the image.
For answering such VQs, people will use different names for the visible colours, or will probably list the colours in varying order, even if the question does not explicitly mention the word `colo(u)r'.

